FLUTE: A Scalable, Extensible Framework for High-Performance Federated Learning Simulations

In this paper we introduce "Federated Learning Utilities and Tools for Experimentation" (FLUTE), a high-performance open-source platform for federated learning research and offline simulations. The goal of FLUTE is to enable rapid prototyping and simulation of new federated learning algorithms at scale, including novel optimization, privacy, and communications strategies. We describe the architecture of FLUTE, enabling arbitrary federated modeling schemes to be realized. We compare the platform with other state-of-the-art platforms and describe available features of FLUTE for experimentation in core areas of active research, such as optimization, privacy, and scalability. A comparison with other established platforms shows speed-ups of up to 42x and savings in memory footprint of 3x. A sample of the platform capabilities is also presented for a range of tasks, as well as other functionality, such as linear scaling for the number of participating clients, and a variety of federated optimizers, including FedAdam, DGA, etcetera.

==> DGA.tex <==


The  $\text{DGA}_{SM}$ algorithm  utilizes the negative training loss coefficients $\mathcal{L}$, as weights $\alpha^{(j)}_t \sim \mathcal{L}(\cdot)$. These weights are normalized when passed through a $\text{Softmax}(\cdot)$ layer,
\begin{equation}
\label{eq:softmax_weights}
    \alpha^{(j)}_T=\exp(\mathcal{-\beta L}^{(j)}_T)/\sum_i{\exp{(-\beta \mathcal{L}^{(i)}_T})}
\end{equation}
where $\beta$ is the temperature of the Softmax function. %The temperature regulates how the weighting of the gradient components is. 
According to Equation~\ref{eq:softmax_weights}, the aggregation weights are smaller for nodes with larger values of the corresponding losses.

The $2^{nd}$ approach is based on Reinforcement Learning. The weights are inferred by a network, trained with RL rewards.  Herein, this approach is called  ``RL Weighting'' (or $\text{DGA}_{RL}$), Algorithm~\ref{alg:RL_Training}.
An agent perceives an ``observation'' from the environment. The rewards  depend on how good the agent's action is, based on a specific, predefined reward policy. This agent takes action in order to optimize the interaction with the environment according to such rewards policy while inducing new states to the system. Then, updated observations and a new reward are acquired based on such a new state. Our approach is based on Active  Reinforcement Learning, where  rewards depend  on the action selected~\cite{EVD08}.  

A neural network $RL(\cdot)$ is trained with Reinforcement Learning to infer the weights, based on the input features $\bf{x}_T^{(j)}$ from each of the $j$-clients. The agent decides on the values of the gradient weights aiming at improving the overall Accuracy (or any other measurement) performance of the model by learning an optimal weighting strategy. The input features consist of the training loss coefficients and the gradient statistics. 


%Translating the training of the network is terms of  Reinforcement Learning (RL), 
The ``actions'', i.e., the weights, are predicted from the results they incur, i.e., the CER on the validation set in every time step $T$. 
%The RL network learns the sequence of actions that lead the ``agent'' to maximize its objective function. 
This reward policy is based on the CER performance, i.e., the ``environment,'' the ``action,'' and ``state'' $s_{T+1}$ is the new aggregated model.%, as in Figure~\ref{fig:RL_schema} from~\cite{SuBa18}. %
In more detail, the ``environment'' in every iteration $T$ is the gradient components $\tilde{g}_T^{(j)}$, the states $s_T$ are described by the input features $\bf{x}^{(j)}_T$, and the action vector $\alpha^{(j)}_T$ is the aggregation weights. The policy is dictated by the output CER performance (on the validation set), %of the updated model~(Equation~\ref{eq:global_update}), 
as  in Alg.~\ref{alg:RL_Training}.
%
The reward policy is based on the CER performance of two different networks that are trained with the aggregated gradients~(\ref{eq:local_gradient}). These two networks are versions of the  same seed model, after training with either the inferred weights or the Softmax-based ones, Equation~\ref{eq:global_update}. Depending on the comparative results, a reward $r_T$ is provided, and the new state $s_{T+1}$ is estimated. The threshold and reward parameters $\theta,\ R$ are part of the reward policy as detailed in Alg.~\ref{alg:RL_Training}.
Herein, the input features $\bf{x}_T^{(j)}$ are the combination of the training loss coefficients (as described above) augmented by the gradient magnitude mean and variance values. The  statistics are estimated on the gradients $\tilde{g}_T^{(j)}$, Eq.~\ref{eq:local_gradient}.  

\vspace{-0.3cm}
\begin{algorithm}[htb]
\caption{Dynamic Gradient Aggregation Based on Reinforcement Learning}
\label{alg:RL_Training}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} $\tilde{g}^{(j)}_T, \bf{x}^{(j)}_T$
    \STATE $RL(\cdot)$: Model Initialization
    \WHILE{Model $w_T^{(s)}$ has not converged}
        \STATE Read the Observations $\bf{x}^{(j)}_T$
        \STATE Estimate Weights $a^{(j)}_T \leftarrow  RL(\bf{x}^{(j)}_T) $
        \STATE Estimate Weights $b^{(j)}_T \leftarrow \text{Softmax}(\bf{x}^{(j)}_T)$, from Equation~\ref{eq:softmax_weights}
    
        \STATE Estimate $\tilde{W}^{(s),a}_T$ and $\tilde{W}^{(s),b}_T$ based on two sets of aggregation weights $a^{(j)}_T, \  b^{(j)}_T$ with Equation~\ref{eq:global_update}
    
        \STATE Estimate $\text{CER}_{a, T},\ \text{CER}_{b, T}$ for the new models $\tilde{W}^{(s),a}_T, \tilde{W}^{(s),b}_T$     %\Comment{Inference on val. set}
        
        \IF {$\text{CER}_{a, T}- \text{CER}_{b, T}>\theta$}
            \STATE $w^{(s)}_{T+1} \leftarrow \tilde{w}^{(s),a}_T$
            \STATE $r_T=R$
        \ELSIF{ $ \text{abs}(\text{CER}_{a, T}- \text{CER}_{b, T}) \leq \theta$ }
            \STATE $w^{(s)}_{T+1} \leftarrow \tilde{w}^{(s),a}_T$
            \STATE $r_T=0.1R$
        \ELSE
            \STATE $w^{(s)}_{T+1} \leftarrow \tilde{w}^{(s),b}_T$
            \STATE $r_T=-R$
        \ENDIF
        \STATE Update model $RL(\cdot)$ on reward $r_T$ 
    \ENDWHILE
\end{algorithmic}
\end{algorithm}


==> FLUTE.tex <==


This section can be found in~\cite{Dimitriadis+21} but it is herein included for the sake of completeness.  

The $j^{th}$ client update runs $t$ iterations with $t\in[0, T_j]$, locally updating the seed model $w^{(s)}_T$ (herein shown using the SDG optimizer, without loss of generality) with a learning rate of $\eta_j$,
\begin{equation}
    w^{(j)}_{t+1}=w^{(j)}_t - \eta_j \nabla  w^{(j)}_t
\label{eq:local_update}
\vspace{-0.12cm}
\end{equation}
where $t$ is the local iterations on $j^{th}$-client, i.e., the client time steps, and  $w_t^{(j)}$ the local model and $w_0^{(j)}\defeq w^{(s)}_T$.

Then, the $j^{th}$ client returns a smooth approximation of the local gradient $\tilde{g}_T^{(j)}$ (over the $T_j$ local iterations and $T$ is the iteration ``time'' on the server side) as the difference between the latest, updated local model $w_{T_j}^{(j)}$ and the previous global model $w^{(s)}_T$ 
\begin{equation}
   \tilde{g}_T^{(j)} = w^{(j)}_{T_j} -   w_T^{(s)}
    \label{eq:local_gradient}
    \vspace{-0.12cm}
\end{equation}
Since estimating the gradients $g_T$ is extremely difficult, hereafter the approximation $\tilde{g}_T^{(j)}$ is used instead.

The gradient samples $\tilde{g}_T^{(j)}$ are weighted and aggregated, as described in~\cite{Dimitriadis+21}
\begin{equation}
   g^{(s)}_T =  \sum_j{\alpha_T^{(j)} \tilde{g}_T^{(j)}}
\label{eq:global_grad}
 \vspace{-0.12cm}
\end{equation}
where $\alpha_T^{(j)}$ are the aggregation weights.

The global model $w^{(s)}_{T+1}$ is updated as in~(\ref{eq:global_grad}) (here also shown using SGD, although not necessary), 
\begin{equation}
   w^{(s)}_{T+1} = w_T^{(s)} - \eta_s g^{(s)}_T.
    \label{eq:global_update}
    \vspace{-0.12cm}
\end{equation}
%where $\alpha_T^{(j)}$ are the weights for the aggregation step, as described in Section~\ref{sec:aggregate}.

The process described in Eq.~\ref{eq:server_training} is a form of ``\emph{Naive Rehearsal}''~\cite{HLRK18, Parisi+18, SPLH17}. Updating the global model may cause drifting - in order to mitigate such drifting, an additional training step is proposed (with held-out data matching the tasks in question) on the server-side, i.e. the model updates are regularized in a direction matching the held-out data. As such,  the model does not diverge too much from the task of interest. 
\begin{equation}
    w^{(s)}_{\tilde{t}+1} = w^{(s)}_{\tilde{t}} - \eta_w \nabla  w_{\tilde{t}}
    \label{eq:server_training}
\end{equation}
%
\begin{algorithm}[!ht]
\caption{Adaptive Federated Optimization}
\label{alg:Hier_Optim}
\begin{algorithmic}[1]
    \STATE {\bfseries Input: }( $w_0^{(s)},\ \bf{x}^{(j)}_T$)
    \WHILE{Model $w_T^{(s)}$ has not converged}
        \FOR{$j\ in\ [0,N]$}
            \STATE Send seed model $w_T^{(s)}$ to $j^{(th)}$ clients 
            \STATE Train local models $w^{(j)}$ in $j^{th}$-node with data $x_T^{(j)}$
            \STATE Estimate a smooth approximation of the local gradients $\tilde{g}_t^{(j)}$ for $j^{th}$-node
            \STATE $j \leftarrow j+1$
        \ENDFOR
        \STATE Estimate weights $\alpha^{(j)}_T$
        \STATE Aggregate weighted sum of gradients, Equation~\ref{eq:global_update}
        \STATE Update global model $w_T^{(s)}$ using aggregated gradient 
        \STATE Update global modal on held-out data, Equation~\ref{eq:server_training}
    \ENDWHILE
\end{algorithmic}
\end{algorithm}
%
The convergence speed of training due to the hierarchical optimization scheme is improved by a factor of $2\times$, without any negative impact in performance. Also, the communication overhead is significantly lower instead of continuously transmitting gradients, as in FedSGD~\cite{McMahan+17}.


DGA is  compared with  FedAdam, $DGA_{SM}$ and $DGA_{RL}$, on the Speech Recognition task, as in Section~\ref{subsec:tasks}. It is shown in literature that FedAdam is much faster than FedAvg in convergence, and as such this experiment is omitted. The results, as in Figure~\ref{fig:Convergence}, show a significant speed-up due to $DGA_{SM}$, of about $3\times$ compared with the FedAdam. The second approach of $DGA_{RL}$ is about 40\% faster than the $DGA_{SM}$, consistent across various tasks.
%
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\textwidth]{mlsys2022style/figures/convergence.png}
    \caption{Convergence of various algorithms on the ASR LibriSpeech Task. Figure extracted from \cite{Dimitriadis+20} and produced using an early version of the FLUTE platform.}
    \label{fig:Convergence}
\vspace{-.4cm}
\end{figure}



==> architecture.tex <==



In the sections below, we distinguish the logical workflow from the physical implementation of FLUTE so that accurate logical simulation can be implemented as efficiently as possible in the physical platform. 

% We distinguish between the logical workflow and physical implementation of FLUTE so that accurate logical simulation can be implemented as efficiently as possible in the physical platform. In the sections below we first discuss  FLUTE logical workflow, followed by a description of its physical implementation.

\subsection{Logical Workflow}
\label{subsec:overview}

%FLUTE has been designed as a scalable framework for rapid prototyping of FL scenarios. As such, it enables researchers with the flexibility to run large-scale experiments,  encouraging them to propose novel FL solutions that address real-world applications. 

FLUTE design is based on a central server architecture, as depicted in Figure~\ref{fig:architecture}.
%
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/flute-architecture.png}
    \caption{Logical architecture of the FLUTE platform }
    \label{fig:architecture}
\end{figure}

The logical workflow performed by FLUTE is: 
%
\begin{enumerate*}[label=(\roman*)]
    \item  Send  an initial global model to clients,
    \item \label{itm:second} Train instances of the global model with locally available data on each client,
    \item Send training information, e.g., adapted models, logits, and/or gradients/pseudo-gradients back to the server, %(encryption is currently under implementation in FLUTE) to the server,
    \item Combine the returned information on the server to produce a new global model,
    \item Optionally, update the global model with an additional server-side  rehearsal step,
    %Updating the global model (optionally with additional server data), and
    \item \label{itm:sixth} Send  the updated global model to the clients,
    \item Repeat Steps~\ref{itm:second} - \ref{itm:sixth} after sampling a new subset of clients for the next training iteration.
\end{enumerate*}



\subsection{FLUTE Implementation}

The distributed nature of FLUTE is based on Python/PyTorch, using \textcolor{blue}{torch.distributed} ~\cite{} as the backbone for communication. A FLUTE job consists of one or more independent nodes, e.g., multi-GPU VMs, running up to K workers, executing tasks assigned by the server. %The tasks typically consist of using clients' data to either update a model or compute metrics. 

\begin{figure}[thb]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/flute_flow.png}
    \caption{FLUTE Execution Flow: The server samples M of the clients and sends them to the K workers. Every time one of the workers finishes processing the client data, it returns the gradient and draws the next client until all clients are processed.
    Figure based on \cite{bonawitz2019towards}, which describes a similar process.}
    \label{fig:mpi}
\end{figure}

During training, the server has the roles of both \emph{orchestrator} and \emph{aggregator}. First, it distributes client-IDs among the workers. The workers, on their turn, process the clients' data to produce new models, and send the models back to the Server. After a number of clients is processed, the server will aggregate all the resulting models, typically into a single global model. Algorithm~\ref{alg:flute} describes in detail this process and Figure~\ref{fig:mpi} exemplifies the execution flow .

\begin{algorithm}[!ht]
\caption{FLUTE Orchestration: $P$ is a Client Pool, which contains data of each client, $N$ is the federation rounds to be executed, and  $K$ is the number of Workers}
\label{alg:flute}
\begin{algorithmic}[l]
    \STATE {\bfseries Server-Side Worker-0:}
    \FOR{ each federated round from 1,2,.. to $N$ }
        \STATE $C$ $\leftarrow$ Sample $M$ clients from $P$
        \FOR{$client$ in $C$}
            \STATE Dispatch model and $client$ to available $worker_k$
        \ENDFOR
        \REPEAT 
            \STATE Wait for $worker_k$ to finish
            \STATE Save pseudo-gradient response from $worker_k$
            \STATE $c$ $\leftarrow$ Sample $client$ from $P$
            \STATE Dispatch model and client data $c$ to $worker_k$
        \UNTIL { all $client$ in $P$ has been processed }
        \STATE Aggregate pseudo-gradients
        \STATE Update model with optimization step
    \ENDFOR
    \STATE 
    \STATE {\bfseries Client-Side Worker-$k > 0$:}
    \STATE Load client and model data
    \STATE Execute Training Procedure
    \STATE Send pseudo-gradient to Worker-0
    \STATE Send Statistics about local training to Worker-0
\end{algorithmic}
\end{algorithm}


Figure~\ref{fig:client_server} illustrates the communication between ``Worker 0/Server" and the remaining workers. The interface between Server and Workers is based on ``messages'', client-IDs and training information. In summary, there are four \emph{messages} that can be passed from server to worker:
\begin{enumerate*}
  \item \texttt{Update}: Creates a copy of the model on the worker. Model is passed from server to worker using MPI.
  \item \texttt{Train}: Triggers the execution of a training step on a worker, for a given client. The resulting model (or pseudo-gradient) is passed from worker to server.
  \item \texttt{Evaluate}: Triggers the execution of an evaluation step in a given client. Resulting metrics are passed from worker to server.
  \item \texttt{Terminate}: Shuts down MPI thread where worker has been instantiated.
\end{enumerate*}
%
\begin{figure}[thb]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/client-server.png}
    \caption{Client-server communication protocol.}
    \label{fig:client_server}
\end{figure}


In contrast to distributed training, any end-node such as smartphones or private Cloud computes can be a client in an FL application. As such, local data on each client stays  within the local storage boundaries and it is never either sent to the server or aggregated with other local data sources. Only (sometimes encrypted~\footnote{Encryption and secure aggregation are not currently implemented in FLUTE - these are security mechanisms which aren't strictly necessary for simulation.}) models or gradients are communicated between servers and clients. %So, local training data cannot be shuffled and/or assigned to any other computing nodes as it is usually done in centralized and/or distributed training, to protect the local privacy of each client.
In this research simulator, all clients are implemented as isolated object instances, and never communicate training data (as part of the FLUTE design, the server can hold all clients' data during these simulations, to optimize communication overheads -- however, this doesn't impact the FL assumptions).


%\subsubsection{FLUTE Orchestration}


%{\mirian
% At each iteration, the orchestrator sends a copy of the model to each worker, samples a number of clients, and then continuously sends their data to workers as they become available. 
 
% During execution, the orchestrator may sample a subset of clients, and may also randomly delay pseudo-gradient updates from some clients to future rounds. Occasionally, the server might also ask the workers to use the client's data not to produce a new model, but to evaluate the current model and produce metrics instead.} {\color{red} Although, it is generally expected that (especially in AzureML) there will be one worker per GPU on each node, FLUTE supports multiple processes per GPU node}.  %Due to networking overhead, it is often faster to run jobs on a single node with 8 or 16 GPUs, rather than on multiple nodes.
%





%A scheme of how the server executes the training rounds at any given iteration is shown on
%Figure \ref{alg:flute}.






==> architecture_2.tex <==
%workshop version

%\subsection{FLUTE Architecture}
%\label{subsec:architecture}



FLUTE design is based on a central server architecture, as depicted in Figure~\ref{fig:client_server}. The logical workflow is: 
%
\begin{enumerate*}[label=(\roman*)]
    \item  Send  an initial global model to participating clients,
    \item \label{itm:second} Train instances of the global model with the locally available data on each client,
    \item Send training information, e.g., updated model parameters, logits (if required), and/or gradients/pseudo-gradients back to the server, %(encryption is currently under implementation in FLUTE) to the server,
    \item Combine the returned information on the server to produce a new global model,
    \item Optionally, update the global model with an additional server-side  rehearsal step,
    %Updating the global model (optionally with additional server data), and
    \item \label{itm:sixth} Send  the updated global model to the subset of clients,
    \item Repeat steps~\ref{itm:second} - \ref{itm:sixth} after sampling a new subset of clients for the next training iteration.
\end{enumerate*}

%
%\begin{figure}[!ht]
%    \centering
%    \includegraphics[width=0.5\textwidth]{MainFolder/figures/architecture_updated_horizontal.png}
%    \caption{FLUTE Logical workflow }
%    \label{fig:architecture}
%\end{figure}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{MainFolder/figures/server-client-pdf.pdf}
    \caption{Client-server communication protocol. At each iteration, the server sends a copy of the global model to each worker, samples a number of clients and asynchronously assigns them to a worker as they become available}
    \label{fig:client_server}
\end{figure*}




%\subsection{FLUTE Implementation}

%A FLUTE job consists of $K$ independent nodes, $K\geq 2$, e.g., multi-GPU VMs, running up to $K$ workers, executing tasks assigned by the server. 
A FLUTE job leverages one or more multi-gpu VMs running up to a total of $K$ worker processes, each executing tasks assigned by the server (Worker 0). The number of workers is decoupled from the number of clients $P$, allowing the platform to scale to millions of clients even when $K\ll P$. During training, the server plays the role of both the \emph{orchestrator} and the \emph{aggregator}. First, it distributes a copy of the global model(s), training data and the list of all the client-IDs among the workers. The workers, on their turn, process the clients' data to produce new models, and send the models back to the server. After a number of clients is processed, the server will aggregate all the resulting models, typically into a single global model. Algorithm~\ref{alg:flute} describes in detail this process and Figure~\ref{fig:mpi} exemplifies the execution flow.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{MainFolder/figures/flute_flow.png}
    \caption{FLUTE Execution Flow: The server samples $\mathcal{N}$ of the clients and sends them to the K workers. Every time one of the workers finishes processing the client data, it returns the gradient and draws the next client until all clients are processed.}
    %{\ddim The figure is based on \cite{bonawitz2019towards}, describing a similar process}.}
    \label{fig:mpi}
\end{figure*}

% TODO: fix or move to appendix
\begin{wrapfigure}{R}{0.50\textwidth}
\begin{minipage}{0.50\textwidth}
%\vspace{-0.8cm}
\begin{algorithm}[H] %[!ht]
\caption{FLUTE Orchestration: $\mathcal{P}$ is a Client Pool, which contains IDs of each client, $P=|\mathcal{P}|$, $M$ is the federation rounds to be executed,  $K$ is the number of Workers, $\mathcal{N}$ is the subset of clients per iteration and $N=|\mathcal{N}|$ the number of clients per iteration}
\small
\label{alg:flute}
\begin{algorithmic}[l]
    \STATE {\bfseries Server-Side Worker-0:}
    \FOR{ each federated round from $1,\dots,M$ }
        \STATE $\mathcal{N}$ $\leftarrow$ Sample $N$ clients from $\mathcal{P}$
%        \FOR{$k\in[0,K-1]$ sample client-ID $c$ from $\mathcal{N}$}
%            \STATE Dispatch model/$c$ to  $worker_k$
%        \ENDFOR
        \REPEAT 
            \STATE Wait for $worker_k$ to finish
            \STATE Save pseudo-gradient response from $worker_k$
            \STATE $c$ $\leftarrow$ Sample client-ID from $\mathcal{C}$
            \STATE Dispatch model and $c$ to $worker_k$
        \UNTIL { all client-IDs $c$ in $\mathcal{N}$ have been processed }
        \STATE Aggregate pseudo-gradients
        \STATE Update model with optimization step
    \ENDFOR
    \STATE 
    \STATE {\bfseries Client-Side Worker-k}, with $\text{k}>0$:
    \STATE Load client and model data
    \STATE Execute local training processes
    \STATE Send pseudo-gradients and statistics about local training to Worker-0
\end{algorithmic}
\end{algorithm}
\end{minipage}
%\vspace{-0.5cm}
\end{wrapfigure}



The distributed nature of FLUTE is based on PyTorch, using torch.distributed package as the communication backbone. The interface between server and workers is based on ``\textit{messages}'', that contain model parameters, client-IDs and training instructions. There are four message-types that can be passed from server to worker:
\begin{enumerate*}
  \item \textbf{\texttt{Update}} creates a copy of the model parameters and learning rate on the worker,
  \item \textbf{\texttt{Train}} triggers the execution of a training step on a worker, for a given client. The resulting model (or pseudo-gradient) is passed from worker to server,
  \item \textbf{\texttt{Evaluate}} triggers the execution of an evaluation step in a given client. Resulting metrics are passed from worker to server,
  \item \textbf{\texttt{Terminate}} shuts down the worker thread.
\end{enumerate*}
%


FLUTE leverages the communication scheme in Figure~\ref{fig:client_server} by loading a local copy of the training data on each worker prior to training,  significantly reducing the traffic communication between server and workers, only sending client indices. In this research simulator, all clients are implemented as isolated object instances, therefore local data on each client stays  within the local storage boundaries and it is never  sent to the server or aggregated with other local data sources. Only metrics, model parameters or gradients are communicated between the server and clients -- these quantities can be encrypted~\footnote{Encryption and secure aggregation are not currently implemented in FLUTE - these are security mechanisms which aren't strictly necessary for simulations.} if necessary.







==> case_study.tex <==



\section{Case Studies}
\label{sec:experiments}

This section provides insights by exploring a variety of features of the FLUTE platform. The list of presented datasets, tasks and experimental results is by no means exhaustive. In this context, we do not present any of the models used since the platform allows training on any architecture currently supported by PyTorch.


\subsection{Sample of Baseline Experiments and Datasets}
\label{subsec:tasks}

We provide  some of the available models/tasks as part of the FLUTE distribution. This list of models and tasks is \textbf{not} exhaustive since the flexibility of the platform allows extensions in models such as GNN's, GBT's and others:
\begin{itemize}
\item \textbf{ASR Task: LibriSpeech}:
FLUTE offers a Speech Recognition template task based on the LibriSpeech task~\cite{PCPK15}. The dataset contains about 1,000 hours of speech from 2,500 speakers reading books. Each of the speakers is labeled as a different client. In one of the ASR task examples, a sequence-to-sequence model was used for training, more details can be found in~\cite{Dimitriadis+20b}. 

\item \textbf{Computer Vision Task: MNIST and EMNIST}:
Two different datasets, i.e.,  the MNIST~\cite{mnist2010} and the EMNIST  \cite{cohen2017emnist} dataset are used for Computer Vision tasks. The EMNIST dataset is a set of handwritten characters and digits captured and converted to $28\times28$ pixel images maintaining the image format and data-structure and directly matching the  MNIST dataset. Among the many splits of EMNIST dataset, we use the ``EMNIST Balanced'',  containing \~132k images with 47 balanced classes.

\item \textbf{NLP Tasks: Reddit}:
Different NLP tasks are supported in FLUTE with 2 use-cases for MLM and next-word prediction using Reddit data~\cite{baumgartner2020pushshift}. The Reddit dataset consists of users' tweets grouped in months when published on the social network. For the use-cases, we use 2 months of Reddit data with 2.2M users.%{\color{red}\textbf{mean length  XX words and XX sentences per user}}. 
The initial/seed models used are based either on HuggingFace or a baseline LM model, as described below. 

\item \textbf{Sentiment Analysis: sent140, IMDb, YELP}:
Sent140~\cite{sent140}, is a sentiment analysis dataset consisting of tweets, automatically annotated from the emojis found in them. The dataset consists of 255k users, with mean length of 3.5 samples per user. IMDb is based on movie reviews of 1012 users providing 140k reviews with 10 rating classes~\cite{imdb2014}. The YELP dataset is based on restaurant review from Yelp and the sentiment label is from 1 to 5~\cite{yelp2015}. It contains 2.5k users with 425k reviews.

\item \textbf{Baseline LM Model}: A baseline LM model is used for most of the experiments in Section~\ref{sec:experiments}. A two-layer GRU with 512 hidden units, 10,000 word vocabulary, and embedding dimension 160 is used for fine-tuning during the FL experiments. The seed  model is pretrained on the Google News corpus \cite{Gu+20}.

\end{itemize}


\subsection{DP Experiments}
\input{MainFolder/dp_expt}



\subsection{Quantization Experiment}
\input{MainFolder/quantization_experiments}





%\subsection{Stale Gradients}
%\label{subsec:stale_grads}
%
%We experimentally verify the theoretical analysis in Appendix~\ref{app:stale_grad} with two different experiments, depending on the percentage of stale clients, 20\% and 50\% of the 1000 clients are stale -- staleness in this experiment equals to 1 cycle. This experiment is based on the next-word prediction task using the Reddit dataset, together with the baseline LM model described in Section~\ref{subsec:tasks}. As suggested, the model still converges to an optimal point in terms of accuracy. However, it takes longer for the case of 50\% to reach a good point in performance. 
%%
%\begin{figure}[!ht]
%    \centering
%    \includegraphics[width=0.5\textwidth]{MainFolder/figures/stale_gradients.png}
%    \caption{Next-word Prediction task: Top-1 Accuracy for Reddit dataset with Staleness or 1 iteration.}
%    %\vspace{-0.4cm}
%    \label{fig:stale}
%\end{figure}


\subsection{Performance for Variable/Different Number of Clients}
\input{MainFolder/scaling.tex}

\subsection{Comparing Optimizers}
\input{MainFolder/opt_expt}



==> communication.tex <==
\subsubsection{FLUTE Communication}
\label{subsec:communication}

During training, the server has both roles of \emph{orchestrating} and \emph{aggregating}. At each iteration, it sends a copy of the model to each worker, samples a number of clients, and then continuously sends their data to workers as they become available. The workers, on their turn, process the clients' data and send the resulting model back to the server. After a number of clients is processed, the server will aggregate all the resulting models, typically into a single global model.
From time to time, the server might also ask the workers to use the client's data not to produce a new model, but to evaluate the current model and produce metrics instead.

In summary, there are four \emph{commands} that can be passed from server to worker:

\begin{itemize}
  \item \texttt{Update}: Creates a copy of the model on the worker. Model is passed from server to worker using MPI.
  \item \texttt{Train}: Triggers the execution of a training step in a given client. Resulting model (or pseudo-gradient) is passed from worker to server.
  \item \texttt{Evaluate}: Triggers the execution of an evaluation step in a given client. Resulting metrics are passed from worker to server.
  \item \texttt{Terminate}: Shuts down MPI thread where worker has been instantiated.
\end{itemize}



\begin{figure}[thb]
    \centering
    \includegraphics[width=0.45\textwidth]{mlsys2022style/figures/client-server.png}
    \caption{Client-server communication protocol.}
    \label{fig:client_server}
\end{figure}


==> compare_table.tex <==
\begin{table*}[!ht]
\resizebox{\textwidth}{!}{
\centering
    \begin{tabular}{lccc}
        \toprule
         & FLUTE & Tensor Flow Federated & PySyft \\
        \midrule
        Framework & PyTorch & Tensorflow & Pytorch \\
        Communication & MPI & NCCL & Homebrew Protocol \\
        Cloud Integration & \cmark & \cmark & \cmark \\
        Server Side Definitions & \cmark & \cmark & \cmark \\
        Dropout & \cmark & \cmark  & \cmark \\
        Support Multiple Federated Optimization Schemes & \cmark & \cmark & \xmark \\
        Scalability & \cmark & \cmark & \xmark \\
        Stale clients & \cmark & \xmark & \xmark \\
        Differential Privacy & Built-in & Not-Native & Built-in \\
        Flexibility & Dynamic & Static & Dynamic \\
        Support Multiple Federated Optimization Techniques & \cmark & \cmark & Limited \\
        \bottomrule
    \end{tabular}
}
\caption{Comparison between FLUTE and Popular Federated Learning Simulation Platforms}
\label{tab:comparison}
\end{table*}	



==> comparison_platform.tex <==
% FLUTE is a framework that allows customized training procedures and complex algorithmic implementations, resulting in a scalable simulator for rapid prototyping of FL environments that addresses a significant real-world problem: to validate the feasibility of novel FL solutions. 

FLUTE allows customized training procedures and complex algorithmic implementations, making it a valuable tool to rapidly validate the feasibility of novel FL solutions, %Thus, FLUTE allows researchers to generate more robust models,
while avoiding the need to deal with complications that production environments present.


To this day, different FL platforms have been proposed, however, most of them have been designed with a specific purpose which limits the flexibility to experiment with complex large-scale FL scenarios in a reasonable amount of time. %Current FL frameworks include a wide variety of tools, but only a few support customized training procedures for experimentation environments. 
Table \ref{tab:targets} shows the most common FL platforms and their main focus.

\begin{table}[!ht]
\vskip -0.1in
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
 Platform & Focus \\
\midrule
FLUTE & FL Research and Simulation \\
Tensor Flow Federated & FL Research and Simulation\\
PySyft & Simulation and Privacy \textcolor{blue}{Privacy *}\\ 
LEAF & Datasets and Metrics \textcolor{blue}{FL Benchmarking *}\\
FedML & Production Oriented \textcolor{blue}{FL Research and Production*} \\
Flower & Production Oriented  \textcolor{blue}{FL Research and Production*}\\
\bottomrule
\end{tabular}
}
\caption{Most common platforms for FL and their Focus}
\vskip -0.1in
\label{tab:targets}
\end{table}

\textcolor{blue}{Mirian: Most production-oriented frameworks allow researchers to work in a simulation environment within the same platform. However, because their architecture is optimized towards implementation, when it comes to simulate complex FL scenarios, they suffer from being limited in the optimization of resources. Table~\ref{tab:nccl-comparison}  shows that FLUTE architecture provides a significant advantage in runtime and memory utilization, leveraging the benefits from NCCL in GPUs, outperforming in some cases 19 times faster.}

Table~\ref{tab:comparison} shows a deeper comparison focusing only on research-dedicated platforms and their main features.

\textcolor{blue}{Mirian: I think Table 8 (old comparison) and the paragraph above should be removed.}

% rsim: moved to before the comparison section header.
% \input{mlsys2022style/compare_table}

In recent years, researchers have made significant efforts to address the challenges FL raises, especially when it comes to setting up FL-friendly environments -- privacy guarantees, time-consuming processes, communication costs and beyond. With FLUTE, some of these challenges are addressed allowing enhanced customization and enabling new research at realistic scales. 
% The motivation behind FLUTE is to spark further FL-related research.

==> comparison_platforms_neurips.tex <==

\section{Comparison with related platforms}
\label{sec:comparison}

FLUTE allows customized training procedures and complex algorithmic implementations in scale, making it a valuable tool to rapidly validate the feasibility of novel FL solutions, while avoiding the need to deal with complications that production environments present. To this day, different FL platforms have been proposed, however, most of them have been designed with a specific purpose limiting their flexibility to experiment with complex large-scale FL scenarios in a reasonable amount of time using limited resources. Table \ref{tab:comparison} shows a detailed comparison of the most common FL platforms features and their main focus.

%\begin{table*}[!ht]
%\centering
%\resizebox{0.5\textwidth}{!}{
%\centering
%    \begin{tabular}{cc}
%    \toprule
%    \multicolumn{1}{c}{Platform} & Focus \\
%    \midrule
%	FLUTE & FL Research and Simulation \\
%	Tensor Flow Federated & FL Research and Simulation\\
%	PySyft & Privacy \\ 
%	LEAF & FL Benchmarking \\
%	FedML & FL Research and Production \\
%	Flower & FL Research and Production\\
%    \bottomrule
%\end{tabular}
%}
%\caption{Most common platforms for FL and their Focus}
%\label{tab:targets}
%\end{table*}	

\begin{table*}[t]
\resizebox{\textwidth}{!}{
\centering
    \begin{tabular}{lccc}
        \toprule
         & FLUTE & FedML (Parrot) & Flower (Simulator) \\
        \midrule
        Focus & Research and Simulation & Research and Production & Research and Production \\
        ML Framework & PyTorch & PyTorch & PyTorch / TensorFlow \\
        Communication Protocols Supported & Gloo,NCCL & SP, MPI & Ray, gRPC \\
        Support Security/Privacy related functions & \cmark & \cmark & \cmark \\
        Support Multiple Federated Optimization Techniques & \cmark & \cmark & \cmark \\
        Flexible and Generic API  & \cmark & \cmark & \cmark \\
        Cloud Integration & \cmark & \cmark & \xmark \\
        Multi-GPU Support & \cmark & \cmark & \xmark \\
        Performance Optimizations & \cmark & \xmark & \xmark \\
        Easily Extensible to Production & \xmark & \cmark & \cmark \\
        %Memory Efficiency & \cmark & \xmark & \xmark \\
        %Scalability & \cmark & \cmark & \xmark \\
        %Stale clients & \cmark & \xmark & \xmark \
        %Differential Privacy & Built-in & Not-Native & Built-in \\
        %Flexibility & Dynamic & Static & Dynamic \\
        %Server Side Definitions & \cmark & \cmark & \cmark \\
        %Dropout & \cmark & \cmark  & \cmark \\

        \bottomrule
    \end{tabular}
}
\caption{Comparison between FLUTE and Popular Federated Learning Simulation Platforms. This analysis is focused on the simulators provided by these platforms only.}
\label{tab:comparison}
\end{table*}	


Some production-oriented frameworks allow researchers to work in a simulation environment using the same platform. However, such frameworks suffer from lack of flexibility and  limited functionality since their architecture is optimized towards productization.
We selected the \textit{FedML} and \textit{Flower} platforms as two of the most representative, based on their number of stars on GitHub.  
%in the optimization of resources because their architecture is optimized towards implementation, when it comes to simulate complex FL scenarios, .

FLUTE architecture provides a significant advantage in runtime and memory utilization, leveraging the benefits when using NCCL in GPUs, the  communication optimization, etc, outperforming all other platforms by $42\times$ in speed and $3\times$ in memory consumption, Tables~\ref{tab:comparison-nccl} and~\ref{tab:gloo-comparison}.


\input{MainFolder/nccl-comparison}

The advantage of FLUTE relies on its ability to asynchronously assign new clients to the workers, as they become available, and receive their outputs. On the other hand, FedML\footnote{FedML Simulator (Parrot) on its release 0.7.303, commit ID 8f7f261f (\url{https://github.com/FedML-AI/FedML/tree/8f7f261f44e58d0cb5a416b0d6fa270b42a91049})} links the number of workers with the number of MPI processes, which is reflected as the number of parallel clients during training. 
FLUTE design allows processing multiple clients per worker decoupling the need for $1:1$ mapping between clients and training processes. 
Another FLUTE strength is that each worker holds a preloaded local copy of the training data, avoiding communication overheads during training as the Server only sends indices of clients to instantiate. An additional comparison of FLUTE with the Gloo backend vs Flower 1.0.0 is presented in Appendix~\ref{app:comparison_details}.

==> comparison_training_details.tex <==


\section{Comparison with different platforms}
\label{app:comparison_details}

To enable the comparisons, the training configurations for the experiments presented in Table~\ref{tab:comparison-nccl} are based on the FedML Benchmarking Recipes~\footnote{FedML Benchmarking Results \url{https://doc.fedml.ai/simulation/benchmark/BENCHMARK_MPI.html}} using the setup and models as detailed in the FedML repository\footnote{FedML Benchmarking Examples \url{https://github.com/FedML-AI/FedML/tree/master/python/examples/simulation/mpi_fedavg_datasets_and_models_example}}. The datasets are also provided by FedML\footnote{FedML Datasets \url{https://github.com/FedML-AI/FedML/tree/master/python/fedml/data}}.
The FLUTE scripts can be found at the \textit{Experiments} folder in the repository. More details about the specific setups are detailed in Table~\ref{tab:nccl-comparison-details}.

\begin{table*}[!ht]
\resizebox{\textwidth}{!}{
\centering
    \begin{tabular}{ccccccccccc}
    \toprule
    Model & Dataset & Algorithm & \# Clients & Clients/round & Batch Size & Client Optim. & lr & Local Epochs & \# Rounds & Test Freq \\
    \midrule
    Log. Regr. & mnist & FedAvg & 1000 & 10 & 10 & SGD & 0.03 & 1 & 100 & 20\\
    CNN & fedmnist & FedAvg & 3400 & 10 & 20 & SGD & 0.1 & 1 & 800 & 50 \\
    ResNet18 & fedcifar100 & FedAvg & 500 & 10 & 20 & SGD & 0.1 & 1 & 4000 & 50\\
    RNN & fedshakespeare & FedAvg & 715 & 10 & 4 & SGD & 0.8 & 1 & 1200 & 50 \\
    \bottomrule
\end{tabular}
}
\caption{Training configuration for FedML Benchmarking}
\label{tab:nccl-comparison-details}
\end{table*}	


%In order to compare CPU performance using Gloo backend , we evaluated the overall time of the job in FLUTE 1.0.0 vs Flower 1.0.0~\footnote{Flower Simulator on its release 1.0.0, commit ID 4e7fad9 -  https://github.com/adap/flower/tree/4e7fad99389a5ee511730841b61f279e3359cb16} in Table~\ref{tab:gloo-comparison} using the same setup for the \textit{"lr mnist"} task described in Table~\ref{tab:nccl-comparison-details}. FLUTE results outperform up to $54\times$ faster than Flower on GPUs given that their simulation capabilities are not optimized for multi-GPU jobs. Also, for the CPU task FLUTE shows a competitive advantage running Gloo backend, over Flower being $9\times$ faster.

The Flower platform seems more efficient when multiple CPUs are employed -- the platform is fairly inefficient by design when multiple GPUs are used  during simulation. To run a fair comparison, we compare the FLUTE CPU performance (using the Gloo backend) against Flower. We evaluate the overall time of the job in FLUTE 1.0.0 vs Flower 1.0.0~\footnote{Flower Simulator on its release 1.0.0, commit ID 4e7fad9 -  https://github.com/adap/flower/tree/4e7fad99389a5ee511730841b61f279e3359cb16}, as in Table~\ref{tab:gloo-comparison} using the same setup for the \textit{"lr mnist"} task described in Table~\ref{tab:nccl-comparison-details}. FLUTE results outperform up to $54\times$ faster than Flower on GPUs given that their simulation capabilities are not optimized for multi-GPU jobs. Also, for the CPU task FLUTE shows a competitive advantage running Gloo backend, over Flower being $9\times$ faster.



\begin{table*}[!ht]
\centering
\resizebox{0.5\textwidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
    \multicolumn{1}{c}{} &\multicolumn{3}{c}{FLUTE 1.0.0} & {Flower 1.0.0} \\
    \multicolumn{1}{c}{} &\multicolumn{3}{c}{Gloo/NCCL} & {gRPC} \\
    \cmidrule{1-5}
     Accelerator & Acc & Time & Acc & Time\\
    \midrule
    CPU & 80 & \textbf{00:03:20}  & 80 & 00:30:14\\
    GPU 2x & 80 & \textbf{00:01:31}  & 80 & 01:21:44 \\
    GPU 4x & 81 & \textbf{00:01:26}  & 79 & 00:56:45\\
    \bottomrule
\end{tabular}
}
\caption{Performance comparison FLUTE 1.0.0 vs Flower 1.0.0 on 4x NVIDIA RTX A6000, AMD EPYC 7V12 64-Core Processor. Test accuracy is reported from the last communication round.  }
\label{tab:gloo-comparison}
\end{table*}	





==> dga_theory.tex <==

The gradient aggregation of Equation~\ref{eq:global_grad}, can be seen as (dropping the subscript $T$)
\begin{equation}
\begin{split}
    \mathbb{E}_p[g^{(s)}]=\int{p(g) g^{(s)} dg} &  \\ 
    =\mathbb{E}_\alpha \left[ \frac{p(g)}{\alpha(g)}g^{(s)} \right] 
    &\simeq \frac{1}{N}\sum_{j=1}^N{\alpha^{(j)}g^{(j)}}    
\end{split}
\end{equation}
where $p(\cdot)$ is the probability density function of the random variable $\mathcal{G}$ and $g^{(s)}$ is the  function mapping gradients to the gradient space $\mathbb{R}^d$, with $d$ the gradient dimension. The mean value of the gradient $g^{(s)}$ can be approximated by the weighted sum of the gradient samples  $g^{(j)}$ for $j=1,\dots,N$ based on the client data, as long as $a^{(j)}~\sim p(g^{(s)})$ and $\alpha^{(j)}\geq0$. Equally, if the training step in the server and clients is considered as a large-batch process then $g^{(s)}\sim\nabla_\theta\mathcal{L}(\cdot)$, as in Section~\ref{subsec:DGA}, and $g^{(j)}$ are samples of the random variable $\mathcal{G}$. 

It is shown, that reducing the variance of the gradient $g^{(s)}$ can improve the convergence speed during training.
In a multi-dimensional space, it is shown that an equivalent criterion of variance minimization is  minimizing the eigenvalues of the Covariance matrix $\Sigma(\cdot)$ of the weighted gradients, or equally $\min_\alpha \Tr(\Sigma(\alpha))$, 
%, where $\alpha$ from Eq.~\ref{eq:global_grad} and $g=\{g^{(j)}\}_{j=1}^N$ are the gradients from the $j^{th}$ clients, Equation~\ref{eq:local_gradient}. 
where $\Sigma(\alpha)$ is a function of the gradient weights $\alpha=\{\alpha^{(j)}\}_{j=1}^N$, and we will minimize the $\Tr\left(\Sigma(\alpha)\right)$ by optimizing these weights~\cite{Alain+16},  

\begin{equation}
    \Tr(\Sigma(\alpha))
    %= \Tr\left(\mathbb{E}_\alpha \left[\left(\frac{p}{\alpha}g^{(s)}-\mu \right) \left(\frac{p}{\alpha}g^{(s)}-\mu \right)^T \right] \right) 
    =\mathbb{E}_\alpha \left[ \norm{\frac{p(g)}{\alpha(g)} \nabla _\theta \mathcal{L}(\cdot)}_2^2\right]-\norm{\mu}_2^2
    \label{eq:orig_sampler}
\end{equation}
where $\mu=\mathbb{E}_p[\nabla _\theta \mathcal{L}(\cdot)]$. Based on Eq.~\ref{eq:orig_sampler}, the optimal weights $\alpha^*$ are given by 
\begin{equation}
    \alpha^*=\frac{1}{Z}p(g)\norm{ \nabla_\theta \mathcal{L}(\cdot)}_2
    \label{eq:optimal_weights}
\end{equation}
where $Z=\int{p(g)\norm{\nabla _\theta\mathcal{L}(\cdot)}_2 dg}$, according to~\cite{Alain+16}. 
\\
\\
\textbf{Proof.}
\begin{equation}
    \begin{split}
        \Tr(\Sigma(\alpha)) &= \Tr\left( \mathbb{E}_\alpha \left[ \left(\frac{p}{\alpha}
         g^{(s)}-\mu\right)\left(\frac{p}{\alpha} g^{(s)}-\mu\right)^T\right] \right) \\
         & =  \Tr\left(  \mathbb{E}_\alpha \left[\left(\frac{p}{\alpha} g^{(s)}\right)\left(\frac{p}{\alpha} g^{(s)}\right)^T\right]-\mu\mu^T\right) \\
         & =  \mathbb{E}_\alpha \left[  \Tr\left( \left(\frac{p}{\alpha} g^{(s)}\right)\left(\frac{p}{\alpha} g^{(s)}\right)^T\right)\right]-\norm{\mu}_2^2 \\
         & =  \mathbb{E}_\alpha \left[  \norm{\frac{p}{\alpha} g^{(s)}}_2^2\right]-\norm{\mu}_2^2
    \end{split}
 \label{eq:theory_analysis}
 \end{equation}
 
 From Jensen's inequality, we get,
\begin{equation}
    \begin{split}
        \mathbb{E}_\alpha \left[  \norm{\frac{p}{\alpha} g^{(s)}}_2^2\right] \geq  \left(  \mathbb{E}_\alpha \left[\norm{(\frac{p}{\alpha} g^{(s)}}_2\right]\right)^2 & \\
         = \left(  \int{\frac{p}{\alpha} \norm{g^{(s)}}_2 dg}  \right)^2  = & \left(  \mathbb{E}_p\left[  \norm{g^{(s)}}_2 \right]  \right)^2 
    \end{split}
 \label{eq:theory_ineq}
 \end{equation}
 when $\alpha, p \geq 0$. Based on Equation~\ref{eq:theory_ineq}, the lower bound for $\Tr(\Sigma(\alpha))$ is $\left(  \mathop{\mathbb{E}}_p\left[  \norm{g^{(s)}}_2 \right]  \right)^2-\norm{\mu}_2$.

 Now, replacing the weights $\alpha$ with the $\alpha^*$ from Equation~\ref{eq:optimal_weights}, we get
 \begin{equation}
    \begin{split}
            \Tr(\Sigma(\alpha^*)) &= \mathbb{E}_{\alpha^*} \left[ \norm{(\frac{p(g)}{\alpha^*} g^{(s)}}_2^2\right]-\norm{\mu}_2^2 \\
            &= \int{\alpha^* \left(\frac{p(g)}{\alpha^*} \right)^2 \norm{g^{(s)}}_2^2 dg}-\norm{\mu}_2^2  \\
            &= \int{ \frac{p^2 Z}{p(g)\norm{ g^{(s)}}_2}  \norm{g^{(s)}}_2^2 dg}-\norm{\mu}_2^2 \\
            &= \left( \mathbb{E}_p\left[  \norm{g^{(s)}}_2 \right]  \right)^2-\norm{\mu}_2
    \end{split}
    \label{eq:theory_optimal_weights}
 \end{equation}
 So, we have proved that $\alpha^*$ provides the optimal solution based on the lower bound estimated in Eq.~\ref{eq:theory_ineq}.
 
 
For a function $h:~\mathcal{G} \to \Re^+$, then the Covariance matrix is given by
\begin{equation}
\begin{split}
    \Tr(\Sigma(\alpha))=&\left( \int p(g)h(g)dg \right)  \\
    &\cdot \left( \int p(g)\frac{\norm{\nabla _\theta\mathcal{L}(\cdot)}_2^2}{h(g)}dg \right)   -\norm{\mu}_2^2
\end{split}
\label{eq:sampler}
\end{equation}



In the case when $p(g^{(s)})$ is not known but we can draw samples, i.e. $g^{(j)}$, from that distribution $p(g^{(s)})$, we have that the weights $\alpha$ are approx. proportional to $p(g^{(s)})h(g^{(s)})$ and
%
%In the case $p(g)$ is not known but when sampling the gradients $g^{(j)}$ from $p(g)$, we can still estimate $\alpha \propto p(g)h(g)$ if 
\begin{equation*}
    \tilde{\alpha}_j=h(g^{(j)}),\ \forall g^{(j)}\in g^{(s)}
\end{equation*}
and after normalizing to unity, $\alpha_j=\tilde{\alpha}_j/\sum_j \tilde{\alpha}_j$. Based on the sampled weights $\alpha_j$, Eq.~\ref{eq:sampler} becomes,
\begin{equation}
        \Tr(\Sigma(\alpha))= \left( \frac{1}{N^2}\sum_{j=1}^N{\frac{\norm{\nabla _\theta \mathcal{L}^{(j)}}_2^2}{\alpha_j}}\right)
    \label{eq:weighted_sampler}
\end{equation}

If we replace $h(g^{(j)})=\exp(-\beta \norm{g^{(j)}})$, then we get a form of the DGA algorithm as described in Section~\ref{subsec:DGA}.

Finally, the analysis is based on $\norm{g^{(j)}}$ but it's safe to assume that $\norm{g^{(j)}}\sim \mathcal{L}^{(j)}(\cdot)$, where $\mathcal{L}^{(j)}(\cdot)$ is the training loss for the $j^{th}$ client, since the client optimizer is SGD (without momentum). This assumption has been experimentally verified, as well.
%% Analysis based on https://arxiv.org/pdf/1511.06481.pdf



==> dp_expt.tex <==


In this experiment, we explore privacy-utility trade-offs in LM training, using the baseline  model described in Section~\ref{subsec:tasks}.  Local differential privacy was applied with $\epsilon$ parameter LDP $\epsilon$. We track the per-client noise across all clients and yield a final global RDP $\epsilon$ after 500 rounds of training.  We express the privacy-utility tradeoff as the ratio of accuracy and RDP $\epsilon$.  Clearly, for a fixed number of training rounds, we achieve better privacy and better accuracy by sampling a larger number of clients. We observe a penalty of about 4.3\% relative to the non-private baseline ($\epsilon=\infty$).

\begin{table}[!ht]
    \centering
    \begin{tabular}{ccccc}
    \toprule
         Clients/Iter. & LDP $\epsilon$ & RDP $\epsilon$ & Acc @1 (\%) & Tradeoff \\ \hline
%         10,000 &  $\infty$ & $\infty$ &  0.217079 \\
%         1,000 &  $\infty$ & $\infty$ &  0.214449 \\
%         10,000 &	1000.0 &	7.658402 &	0.203008 \\
%         10,000 &	750.0	& 3.651467 &	0.202566 \\
%         10,000 &	500.0  &	1.414313 &	0.199535 \\
%         1,000 &	1000.0	& 79.701151 &	0.194482 \\
%         1,000 &	750.0	& 38.277433	& 	0.188497 \\
%         1,000	& 500.0	 & 12.552293	&	0.180342 \\
%         10,000 &	100.0 &	0.108212 &	0.172002 \\
%         1,000	& 100.0 &	0.333154	&	0.147939 \\ \hline
10,000 & 100 & 0.108 & 17.20 & 0.00172\\ 
1,000 & 100 & 0.333 & 14.80 & 0.00148\\ 
10,000 & 500 & 1.41 & 20.00 & 0.000399\\ 
1,000 & 500 & 12.6 & 18.00 & 0.000361\\ 
10,000 & 750 & 3.65 & 20.30 & 0.00027\\ 
1,000 & 750 & 38.3 & 18.80 & 0.000251\\ 
10,000 & 1,000 & 7.66 & 20.30 & 0.000203\\ 
1,000 & 1,000 & 79.7 & 19.40 & 0.000194\\ 
10,000 & inf & inf & 21.70 & 0.0\\ 
1,000 & inf & inf & 21.40 & 0.0  \\
\bottomrule

    \end{tabular}
    \caption{Next-word prediction: Results comparing language model accuracy and privacy for various client sampling and LDP $\epsilon$ parameters. All experiments trained for 500 rounds. Trade-off is defined as the ratio of accuracy and RDP $\epsilon$}
    \label{tab:dp_expt}
\end{table}

==> dropout_stale.tex <==


%\subsection{Dropout and Stale Clients}
%\label{subsec:dropout}

The FLUTE platform offers flexibility when sampling the participating clients from the pool of candidates. A range in the number of clients can be given, fluctuating between the two ends. This can be seen as ``\textit{client dropouts}'', where a number of clients can be randomly discarded. Since the default optimization pipeline is based on DGA, as in Section~\ref{subsec:fed_optimizers}, the learning rate can be  adjusted accordingly.

Similar to the dropout functionality, FLUTE offers an option of delaying the contributions of random clients rather than discarding the corresponding gradients. The system can introduce a 1-step ``staleness'' to the system by randomly delaying a subset of the clients by 1 iteration. The convergence analysis for the stale gradients scenario is held in  Appendix~\ref{app:stale_grad}. As shown, the error introduced due to staleness is upper bounded. As such, there is theoretical guarantee that the model will finally converge. The theoretical conclusions are experimentally verified using FLUTE, as shown in Figure~\ref{fig:stale}.





==> features.tex <==

% The main goal of FLUTE is to be a scalable framework for rapid prototyping, encouraging researchers to propose novel FL solutions that address real-world applications, under the following axes:
% \begin{itemize}
%     \item Scalability: Capacity to processs many thousands of clients on any given round. FLUTE allows to run large-scale experiments using up to 10,000 clients with reasonable turn-around time, since scale is a critical factor in understanding  practical metrics such as convergence and privacy-utility trade-offs.
%     \item Flexibility: Allow for any combination of model, dataset and optimizer. FLUTE supports diverse FL configurations, including some of the state-of-the-art algorithms such as DGA, FedAdam and FedAvg, with Pytorch being the framework of choice for implementing the training pipelines.
%     \item Expandable: Allow the end users to easily plug in customized/new techniques like differential privacy or gradient quantization, transfer learning and personalization. FLUTE provides an open architecture allowing the incorporation of new algorithms in a straightforward fashion. 
%     %Additionaly, FLUTE set of tools to run offline experiments, some of the already implemented tools are listed below. 
%     %\item Versatility: The open architecture allows new reserch to be incorporated in a straightforward fashion. FLUTE provides a set of tools to run offline experiments, some of the already implemented tools are listed below. 
% \end{itemize}
% %
% The current FLUTE implementation provides the best-in-class communication speed, outperforming all other experimental platforms by $<40\times$ speed-ups, as shown in Section~\ref{sec:comparison}.





FLUTE provides a range of  built-in functionality while the implemented state-of-the-art algorithms cover important areas in FL. In this section we discuss federated optimization, differential privacy, bandwidth efficiency, personalization and computing resource capablities of FLUTE.

\textbf{Federated Optimization}: FLUTE  already supports a range of federated optimizers by adjusting the gradient aggregation process, and the server-side optimizers,  making FedAvg~\cite{McMahan+17}, FedYogi or FedAdam~\cite{Reddi+20}, and DGA~\cite{Dimitriadis+20, Dimitriadis+21}, straightforward to apply. Also, the FLUTE client scaling capabilities are enhanced by switching to large-batch optimizers on the server-side, like LAMB~\cite{You+20}, and LARS~\cite{YGG17}, validated by the experimental evidence, shown in Appendix~\ref{sec:experiments}.

\textbf{Differential Privacy}: In FLUTE, either local or global DP can be used, depending on whether the clients or the server are responsible for doing the clipping and noise-addition. In both cases, this step is directly applied on the pseudo-gradients, i.e., the difference between current and previous weights after each user's data is processed. The pseudo-gradients are re-scaled so that their norm is at most $C$, ensuring the norm of the difference between any two of them (the sensitivity) is bounded. We typically use Gaussian noise, with variance $\sigma^2 = 2 \log \left(\frac{1.25}{\delta}\right) \frac{C^2}{\epsilon^2}$ picked so that the aggregation is at most $(\epsilon, \delta)$-DP w.r.t. each client. In the case of DGA~\cite{Dimitriadis+20}, the aggregation weights also go through the same procedure, since they are data-dependent.

\textbf{Bandwidth Optimization}: We have incorporated an approach similar to that of~\cite{alistarh2017qsgd}. At each layer of the neural network, we first get the dynamic range of the gradient components, and then create a histogram of $2^B$ bins between these two values. Next, we replace each gradient component by the label of the closest bin. That way, we need just to communicate the bin indices, together with the  min. and max. values. Besides gradient compression and quantization, We also in the process of incorporating FL-algorithms with different model architectures~\cite{Cho+22} and the use of adapters in NLU tasks, achieving even further bandwidth compression.

\textbf{Computing Resources}: AzureML (AML)~\cite{pmlr-v50-azureml15} is the preferred computing FLUTE environment  for staging, executing, tracking, and summarizing the FL experiments. %AML provides Kubernetes services for running containerized workflows on targeted computing nodes, including multi-GPU nodes. 
FLUTE has a native AML integration included for job submissions, allowing the users to use the built-in CLI or web interface for job/experiment tracking, and for visualization purposes. While FLUTE needs only the experiment-related configurations,  AML expects the computing environment parameters in a configuration file, such as target, cluster, code, etc. %AML expects two configuration files when submitting jobs: the first contains all the computing environment parameters, e.g., target, cluster, code, and the second is the  experiment-related configurations. %The models and logs can be downloaded to a local machine. AML also enables tracking all the jobs, allowing to rerun crashed jobs, analyze metrics and abort any job in progress. 
Besides AML, FLUTE can also run seamlessly on stand-alone devices, such as laptop and desktop machines (like those used for Section~\ref{sec:comparison}), using the local GPUs if/when available. 




==> fedAvg.tex <==


\subsection{Federated Learning -- FedAvg}
\label{subsec:fedAvg}

The ``Federated averaging'' (FedAvg) algorithm,~\cite{KMR15, McMahan+17} is the first and perhaps the most widely used FL training algorithm. The server samples $\mathcal{M}_T\subset \mathcal{N}$  of the available $\mathcal{N}$ devices and sends the model $\textbf{w}^{(s)}_T$ at that current iteration $T$. Each client $j$, $j\in \mathcal{M}_T$ has a version of the model $\textbf{w}^{(j)}_T$, where it is locally updated with the segregated local data. The size of the available data $\mathcal{D}^{(j)}_T$,  per iteration $T$ and client $j$, is expected to differ and as such, $N^{(j)}_T=|\mathcal{D}^{(j)}_T|$ is the size of processed local training samples. After running $\mathcal{E}$ steps of SGD, the updated model $\hat{\textbf{w}}^{(j)}_T$ is sent back to the server. The new model $\textbf{w}_{T+1}$ is given by
\begin{equation}
    \textbf{w}_{T+1} \leftarrow \frac{1}{\sum_{j\in\mathcal{M}_T} {N^{(j)}_T}}\sum_{j\in\mathcal{M}_T}{N^{(j)}_T \hat{\textbf{w}}^{(j)}_T}
\label{eq:fedavg}
\end{equation}
The server-side model in iteration $T+1$ is a weighted average of the locally updated models of the previous iteration. 

Despite some drawbacks like lack of fine-tuning or annealing of a global learning rate,  FedAvg is the baseline aggregation approach in FLUTE, based on its popularity.



==> fed_optimizers.tex <==



\subsection{Adaptive Optimization}
\label{subsec:FLUTE}

The FedAvg algorithm, although the golden standard in FL training, presents several drawbacks~\cite{zhao2018federated}. A different family of learning algorithms, ``Adaptive Federated Optimizers'' has been proposed to address  them~\cite{Reddi+20, Dimitriadis+20, LSTS18}, where the clients return pseudo-gradients instead of models.  
%Mini-batch optimization methods, extending classical stochastic methods to process multiple data points in parallel, have emerged as a popular paradigm for FL~\cite{LSTS18}. Approaches like  ``Federated Averaging'' (FedAvg)~\cite{KMR15}, a method based on averaging local models after stochastic gradient descent (SGD) updates, are often considered as the golden-standard approach. FedAvg is shown to generalize well while  improving performance in terms of speed-ups. Lately, ``Generalized FedAvg'' was presented in~\cite{Reddi+20, Leroy+19},  with similarities to the proposed hierarchical optimization method.

The training process consists of two optimization steps: first, on the client-side using a stateless optimizer for local SGD steps, and then on the server-side with a ``global'' optimizer utilizing the aggregated gradient estimates. The two-level optimization provides both speed-ups in convergence rates due to the second optimizer on the server, and improved control over the training by adjusting the learning rates. In addition, scaling in the number of clients becomes straightforward by adjusting the server-side optimizer. The proposed algorithm DGA,~\cite{Dimitriadis+21}.%, is shown to converge to a better optimum, faster than other federated algorithms and the centralized training method BMUF\footnote{Anecdotal in-house validation runs based on the number of iterations till convergence.}, after data volume normalization.

The FLUTE system provides support for this group of federated optimizers by adjusting the gradient aggregation weights, and the server-side optimizers, as in Appendix~\ref{app:adaptive_optim} and~\cite{Dimitriadis+20, Dimitriadis+20b, Dimitriadis+21}, making FedYogi, FedAdam~\cite{Reddi+20}, and DGA,~\cite{Dimitriadis+20, Dimitriadis+21}, rather straightforward to apply. Also, the FLUTE client scaling capabilities are enhanced by switching to large-batch optimizers on the server-side, like LAMB~\cite{You+20}, and LARS~\cite{YGG17}, validated by the experimental evidence, shown in Section~\ref{sec:experiments}.





==> quantization_experiments.tex <==
In Table \ref{tab:quant},  the accuracy for a next-word-prediction task is shown, on the Reddit dataset and the baseline LM model described in Section~\ref{subsec:tasks},  while using different values of quantization $B$. As expected, using less bits, while training for the same number of epochs, leads to decreased performance in terms of accuracy.

\begin{table}[!ht]
\center
\label{tab:quant}
%\vskip 0.15in
\begin{tabular}{lccc}
\toprule
 & Quant. (bits) & Acc @1 (\%) & Rel. Imprv. (\%) \\
\midrule
Seed Model          & N/A           &  9.83 & (56.62) \\
SST                 & N/A           & 22.30 & (1.59)        \\
\midrule
FL Train.           & 32            & 22.70 & 0 \\
                    & 10            & 22.40 & (1.32) \\
                    &  8            & 22.20 & (2.25) \\
                    &  4            & 21.30 & (5.87) \\
                    &  3            & 18.80 & (17.21) \\
                    &  2            & 17.80 & (21.58) \\
\bottomrule
\end{tabular}
\caption{Next-word prediction task: Top-1 accuracy after gradient quantization. The number of bits per gradient coefficient varies $2-32$.}
%\vskip -0.18in
\end{table}

We have also done experiments varying the sparsity level, while keeping the quantization constant at 8 bits, cf. Table \ref{tab:sparse}. In this particular experiment, we had gains in bandwidth of up to 16x with no significant change in performance. Error compensation techniques \cite{strom2015scalable} could be attempted in order to increase the performance at higher sparsity levels. The difference in performances for the case of 8-bit quantization level in Tables~\ref{tab:quant} and~\ref{tab:sparse} is due to noise during the training process.

\begin{table}[!ht]
\center
\label{tab:sparse}
%\vskip 0.15in
\begin{tabular}{ccc}
\toprule
 \% Sparsity & Gain in Bandwidth & Acc @1 (\%) \\
\midrule
0.0 & 4x & 22.60 \\
75.0 & 16x & 21.70 \\
95.0 & 80x & 19.00 \\
99.0 & 400x & 17.70 \\
\bottomrule
\end{tabular}
\caption{Performance obtained by varying sparsity level on gradients while keeping quantization fixed at 8 bits -- gains in bandwidth are relative to standard 32 bits gradient. The performance reported is the best one over 5000 iterations, with 1000 clients being processed at each iteration.}
%\vskip -0.1in
\end{table}


